CLIC: Curriculum Learning and Imitation for object Control in non-rewarding environments

In this paper we study a new reinforcement learning setting where the environment is non-rewarding, contains several possibly related objects of various controllability, and where an apt agent Bob acts independently, with non-observable intentions. We argue that this setting defines a realistic scenario and we present a generic discrete-state discrete-action model of such environments. To learn in this environment, we propose an unsupervised reinforcement learning agent called CLIC for Curriculum Learning and Imitation for Control. CLIC learns to control individual objects in its environment, and imitates Bob's interactions with these objects. It selects objects to focus on when training and imitating by maximizing its learning progress. We show that CLIC is an effective baseline in our new setting. It can effectively observe Bob to gain control of objects faster, even if Bob is not explicitly teaching. It can also follow Bob when he acts as a mentor and provides ordered demonstrations. Finally, when Bob controls objects that the agent cannot, or in presence of a hierarchy between objects in the environment, we show that CLIC ignores non-reproducible and already mastered interactions with objects, resulting in a greater benefit from imitation.

==> preamble.tex <==
\usepackage{amssymb}  % assumes amsmath package installed
\usepackage{hyperref}
\usepackage{ucs}
\usepackage{comment}
\usepackage{amsmath}
%\usepackage{fancybox}%fait des boites
\usepackage{pbox}%fait des boites
\usepackage{tcolorbox}
\usepackage{caption}
\usepackage{capt-of}
%\usepackage{subcaption} % incompatible with subfig
%\usepackage[numbers]{natbib}
\usepackage{bm}
\usepackage{graphicx}

\usepackage{array}
\usepackage{multirow}
\usepackage{colortbl}
\usepackage{tikz}
\usepackage{xspace}
\usepackage[caption=false,font=footnotesize]{subfig}
%\usepackage{apalike}
%\usepackage{cite}

\renewcommand{\cite}{\citep}

%%% Math commands
\def\bbbr{{\rm I\!R}}
\def\bbbe{{\rm I\!E}}
\newcommand{\R}{{\bbbr}{}}
\newcommand{\Esp}{{\bbbe}{}}
\renewcommand\Pr{P} % probability
\newcommand\esper[2]{\underset{#1}{\mathbb{E}} \left[#2\right]} % expectation
\newcommand\espernosubstack[2]{\mathbb{E}_{#1} \left[#2\right]} % expectation, without substacking #1
\newcommand\espernobr[1]{\underset{#1}{\mathbb{E}}} % expectation, without brackets
\newcommand\mymax[2]{\textmd{max}_{#1} ~ #2} % max
\newcommand\argmax[2]{\textmd{argmax}_{#1} ~ #2} % argmax
\newcommand\argmin[2]{\textmd{argmin}_{#1} ~ #2} % argmin
\newcommand\trace{\textmd{Tr}} % trace operator
\newcommand\erf{\textmd{erf}} % error function
\newcommand\diag{\textmd{diag}} % diagonal matrix
\newcommand\asinh{\textmd{asinh}} % arcsinh
\newcommand\KL[2]{D_{KL}\left(#1\|#2\right)} % Kullback-Leibler divergence
\newcommand\Id{\mat{I}}% identity matrix
\newcommand{\rbd}{{\sc rbd}\xspace}
\newcommand{\rbfn}{{\sc rbfn}\xspace}
\newcommand{\rbfns}{{\sc rbfn}s\xspace}
\newcommand{\vips}{{\sc vips}\xspace}
\newcommand{\reps}{{\sc reps}\xspace}
\newcommand{\creps}{{\sc creps}\xspace}
\newcommand{\hireps}{{\sc hireps}\xspace}
\newcommand{\aaac}{{\sc a3c}\xspace}
\newcommand{\offpac}{{\sc offpac}\xspace}
\newcommand{\reinforce}{{\sc reinforce}\xspace}
\newcommand{\retrace}{{\sc retrace}\xspace}
\newcommand{\blackdrops}{{\sc black-DROPS}\xspace}
\newcommand{\rock}{{\sc rock}$^*$\xspace}
\newcommand{\ddpg}{{\sc ddpg}\xspace}
\newcommand{\naf}{{\sc naf}\xspace}
\newcommand{\qprop}{{\sc Q-prop}\xspace}
\newcommand{\acer}{{\sc acer}\xspace}
\newcommand{\pgql}{{\sc pgql}\xspace}
\newcommand{\ipg}{{\sc ipg}\xspace}
\newcommand{\cmaes}{{\sc cma-es}\xspace}
\newcommand{\cma}{{\sc cma}\xspace}
\newcommand{\nes}{{\sc nes}\xspace}
\newcommand{\xnes}{x{\sc nes}\xspace}
\newcommand{\pepg}{{\sc pepg}\xspace}
\newcommand{\rwr}{{\sc rwr}\xspace}
\newcommand{\crkr}{{\sc crkr}\xspace}
\newcommand{\gpomdp}{{\sc g(po)mdp}\xspace}
\newcommand\cems{\textsc{cem}s\xspace}
\newcommand\cem{\textsc{cem}\xspace}
\newcommand{\trpo}{{\sc trpo}\xspace}
\newcommand{\ppo}{{\sc ppo}\xspace}
\newcommand{\gps}{{\sc gps}\xspace}
\newcommand{\nac}{{\sc nac}\xspace}
\newcommand{\enac}{e{\sc nac}\xspace}
\newcommand{\inac}{i{\sc nac}\xspace}
\newcommand{\sac}{{\sc sac}\xspace}
\newcommand{\acktr}{{\sc acktr}\xspace}
\newcommand{\ilqg}{i{\sc lqg}\xspace}
\newcommand{\svg}{{\sc svg}\xspace}
\newcommand{\power}{{\sc PoWER}\xspace}
\newcommand{\pilco}{{\sc pilco}\xspace}
\newcommand{\PIBB}{{\sc pi$^{\mbox{\tiny BB}}$}\xspace}
\newcommand{\picma}{{\sc pi$^2$-cma}\xspace}
\newcommand{\pis}{{\sc pi$^{2}$}\xspace}
\newcommand{\ann}{{\sc ann}\xspace}
\newcommand{\anns}{{\sc ann}s\xspace}
\newcommand{\mlps}{{\sc mlp}s\xspace}
\newcommand{\mlp}{{\sc mlp}\xspace}
\newcommand{\rbf}{{\sc rbf}\xspace}
\newcommand{\lwpr}{{\sc lwpr}\xspace}
\newcommand{\nipals}{{\sc nipals}\xspace}
\newcommand{\cad}{{\sc cad}\xspace}
\newcommand{\lcs}{{\sc lcs}\xspace}
\newcommand{\lcss}{{\sc lcs}s\xspace}
\newcommand{\xcsf}{{\sc xcsf}\xspace}
\newcommand{\QR}{{\sc qr}\xspace}
\newcommand{\RR}{{\sc rr}\xspace}
\newcommand{\xcs}{{\sc xcs}\xspace}
\newcommand{\moe}{{\sc m}o{\sc e}\xspace}
\newcommand{\gmr}{{\sc gmr}\xspace}
\newcommand{\gmm}{{\sc gmm}\xspace}
\newcommand{\gmms}{{\sc gmm}s\xspace}
\newcommand{\dmps}{{\sc dmp}s\xspace}
\newcommand{\mdps}{MDPs\xspace}
\newcommand{\ilogmr}{{\sc ilo-gmr}\xspace}
\newcommand{\kdtrees}{{\em kd-trees}\xspace}
\newcommand{\libsvm}{{\sc libsvm}\xspace}
\newcommand{\svd}{{\sc svd}\xspace}
\newcommand{\rmrc}{{\sc rmrc}\xspace}
\newcommand{\nmse}{{\sc nmse}\xspace}
\newcommand{\nmae}{{\sc nmae}\xspace}
\newcommand{\imlm}{{\sc imlm}\xspace}
\newcommand{\mae}{{\sc mae}\xspace}
\newcommand{\ga}{{\sc ga}\xspace}
\newcommand{\pls}{{\sc pls}\xspace}
\newcommand{\ls}{{\sc ls}\xspace}
\newcommand{\rl}{RL\xspace}
\newcommand{\drl}{deep RL\xspace}
\newcommand{\Drl}{Deep RL\xspace}
\newcommand{\dqn}{{\sc dqn}\xspace}
\newcommand{\rls}{{\sc rls}\xspace}
\newcommand{\krls}{{\sc krls}\xspace}
\newcommand{\rfrls}{{\sc rfrls}\xspace}
\newcommand{\irfrls}{i{\sc rfrls}\xspace}
\newcommand{\issgpr}{i{\sc ssgpr}\xspace}
\newcommand{\rgls}{{\sc rgls}\xspace}
\newcommand{\krgls}{{\sc krgls}\xspace}
\newcommand{\lwr}{{\sc lwr}\xspace}
\newcommand{\lwpls}{{\sc lwpls}\xspace}
\newcommand{\lgpr}{{\sc lgp}\xspace}
\newcommand{\nusvr}{$\nu$-{\sc svr}\xspace}
\newcommand{\losvr}{{\sc l}o{\sc svr}\xspace}
\newcommand{\svr}{{\sc svr}\xspace}
\newcommand{\svm}{{\sc svm}\xspace}
\newcommand{\svms}{{\sc svm}s\xspace}
\newcommand{\lssvm}{{\sc ls-svm}\xspace}
\newcommand{\sogp}{{\sc sogp}\xspace}
\newcommand{\rfwr}{{\sc rfwr}\xspace}
\newcommand{\soms}{{\sc som}s\xspace}
\newcommand{\som}{{\sc som}\xspace}
\newcommand{\gpr}{{\sc gpr}\xspace}
\newcommand{\ema}{{\sc em}\xspace}
\newcommand{\ofl}{off-line\xspace}
\newcommand{\onl}{on-line\xspace}
\newcommand{\Ofl}{Off-line\xspace}
\newcommand{\Onl}{On-line\xspace}
\newcommand{\ofp}{off-policy\xspace}
\newcommand{\onp}{on-policy\xspace}
\newcommand{\td}{temporal difference\xspace}
\newcommand{\epse}{episodic policy search\xspace}
\newcommand{\epsa}{episodic-sample\xspace}
\newcommand{\epsas}{episodic-samples\xspace}
\newcommand{\ssa}{step-sample\xspace}
\newcommand{\rwa}{reward-weighted averaging\xspace}
\newcommand{\ssas}{step-samples\xspace}
\newcommand{\edas}{{\sc EDA}s\xspace}
\newcommand{\pse}{policy search\xspace}
\newcommand{\Pse}{Policy search\xspace}
\newcommand{\ngo}{natural gradient optimization\xspace}
\newcommand{\Ngo}{Natural gradient optimization\xspace}
\newcommand{\vgo}{vanilla gradient optimization\xspace}
\newcommand{\Vgo}{Vanilla gradient optimization\xspace}
\newcommand{\pid}{$\mathcal{PID}$\xspace}
\newcommand{\pd}{$\mathcal{PD}$\xspace}
\newcommand{\sqp}{{\sc sqp}\xspace}
\newcommand{\gep}{{\sc gep}\xspace}
\newcommand{\geps}{{\sc gep}s\xspace}
\newcommand{\qp}{{\sc qp}\xspace}
\newcommand{\roll}{rollout\xspace} % discount factor
\newcommand{\rolls}{rollouts\xspace} % discount factor

\newcommand{\robotcub}{{\sc RobotCub}\xspace}
\newcommand{\atr}{{\sc atr}\xspace}
\newcommand{\sarsa}{{\sc Sarsa}\xspace}
\newcommand{\ql}{{\sc q-learning}\xspace}
\newcommand{\barrett}{{\sc Barrett}\xspace}
\newcommand{\icub}{{\sc iCub}\xspace}
\newcommand{\james}{{\sc James}\xspace}

\newcommand{\mymath}[1]{\ensuremath{#1}\xspace}
\newcommand{\mymathbf}[1]{\mymath{\mathbf{\boldsymbol{#1}}}}
\newcommand{\covar}{\mymathbf{\Sigma}}
\newcommand{\vtheta}{\mymathbf{\theta}}

\renewcommand{\vec}[1]{\mymathbf{#1}}
\newcommand{\mat}[1]{\mymathbf{#1}}
%\newcommand{\eps}{\vec{\epsilon}}

\newcommand{\varinit}{\mymath{\covar^{\mbox{\scriptsize init}}}}

\newcommand{\mX}{\mat{X}}
\newcommand{\mG}{\mat{G}}
\newcommand{\mF}{\mat{F}}
\newcommand{\vomega}{\vec{\omega}}
\newcommand{\Vomega}{\vec{\Omega}}
\newcommand{\vs}{\vec{s}}
\newcommand{\vo}{\vec{o}}
\newcommand{\vu}{\vec{u}}
\newcommand{\vx}{\vec{x}}
\newcommand{\vw}{\vec{w}}
\newcommand{\vj}{\vec{j}}
\newcommand{\vphi}{\vec{\phi}}
\newcommand{\VO}{\mathcal{O}}
\newcommand{\U}{\mathcal{U}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\E}{\mathcal{E}}
\newcommand{\T}{\mathcal{T}}

\newcommand{\f}{\mymath{f}}
\newcommand{\inpu}{\vec{\phi}}
\newcommand{\Inpu}{\mymath{\Phi}}
\newcommand{\vinpu}{\mymath{\tilde{\vec{\phi}}}}
\newcommand{\Vinpu}{\mymath{\tilde{\Phi}}}
\newcommand{\vnabla}{\mymath{\tilde{\nabla}_{\vinpu}}}
\newcommand{\vf}{\mymath{\tilde{\f}}}

\newcommand{\hatf}{\mymath{\hat{\f}}}
\newcommand{\hatj}{\mymath{\hat{J}}}
\newcommand{\hatq}{\mymath{\hat{Q}}}
\newcommand{\hatv}{\mymath{\hat{V}}}
\newcommand{\hatu}{\mymath{\hat{U}}}

\newcommand\wi[1]{$\circ$}
\newcommand\bu[1]{$\bullet$}
\newcommand\ot[1]{$\star$}
\newcommand\spa[1]{$\spadesuit$}
\newcommand\dn[1]{.}

\newcommand\partielle[2]{\frac{\partial #1}{\partial #2}} % partial derivative

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=1pt] (char) {\tiny #1};}}

\newcommand{\fk}{{$\mathcal{FK}$}\xspace}

%%% MDP and RL specific commands
\newcommand\pol{\pi} % policy
\newcommand\Pol{\Pi} % policy-space
\newcommand{\params}{{\mymathbf{\theta}}\xspace} % policy parameters (vector)
\newcommand{\Params}{\mymath{\Theta}}
\newcommand{\disc}{\gamma} % discount factor


\newenvironment{definition}{{\bf Definition:}}{\par}
\newenvironment{remark}{{\bf Remark:}}{\par}

\newcounter{cbox} \setcounter{cbox}{0}
\newcommand{\cbox}{\arabic{cbox}}
\newenvironment{mybox}[2]{\refstepcounter{cbox}\begin{tcolorbox}[title=Box \cbox: #1]\label{#2}\par}{\end{tcolorbox}}

\newcounter{cmes} \setcounter{cmes}{0}
\newcommand{\cmes}{\arabic{cmes}}
\newenvironment{mymes}[1]{\begin{tcolorbox}[colback=red!10!white]\refstepcounter{cmes}{\bf Message \cmes:}\label{#1}}{\end{tcolorbox}}

\newenvironment{myAlgo}[2]{
  \refstepcounter{algorithm}
    \parbox{\linewidth}{%
    \hrule
    \hrule
    \noindent\strut\textbf{Algorithm \thealgorithm} #1
    \hrule
}\hfil\vskip0em%
\label{#2}
  }
  
\usepackage{algorithmic}
\usepackage{algorithm} 

\makeatletter
\newcounter{algorithmbis}
\setcounter{algorithmbis}{0}
\renewcommand{\thealgorithmbis}{\thesection.\arabic{algorithmbis}}
\def\algorithmbis{\@ifnextchar[{\@algorithmbisa}{\@algorithmbisb}}
\def\@algorithmbisa[#1]{%
  \refstepcounter{algorithmbis}
  \trivlist
  \leftmargin\z@
  \itemindent\z@
  \labelsep\z@
  \item[\parbox{\linewidth}{%
    \hrule
    \hrule
    \noindent\strut\textbf{Algorithm \thealgorithmbis} #1
    \hrule
  }]\hfil\vskip0em%
}
\def\@algorithmbisb{\@algorithmbisa[]}
\def\endalgorithmbis{\hfil\vskip-1em\hrule\endtrivlist}
\makeatother

\definecolor{myred}{rgb}{0.8,0,0}
\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{myblue}{rgb}{0,0,0.7}
\newcommand{\todo}[1]{\textcolor{myred}{\fbox{\bf Todo:}{\em #1}}}
\newcommand{\todolater}[1]{\textcolor{myblue}{\fbox{\bf Todo:}{\em #1}}}
\newcommand{\todiscuss}[1]{\textcolor{mygreen}{\fbox{\bf To discuss:}{\em #1}}}

